DP-Sync: Hiding Update Patterns in Secure Outsourced Databases with Differential Privacy

In this paper, we have introduced a new type of leakage associated with modern encrypted databases called update pattern leakage. We formalize the definition and security model of DP-Sync with DP update patterns. We also proposed the framework DP-Sync, which extends existing encrypted database schemes to DP-Sync with DP update patterns. DP-Sync guarantees that the entire data update history over the outsourced data structure is protected by differential privacy. This is achieved by imposing differentially-private strategies that dictate the data owner's synchronization of local~data.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> outcache.tex <==
\draft{
\section{Outsourcing the Local Cache}

{\bf The contents of this chapter are draft only}\\

Just putting together some key ideas about how to outsource the cache to the \cs, the motivations, and sketch analysis of the accuracy and performance.

\boldparagraph{Motivations}:
\begin{itemize}
    \item when the \user is only able to have $O(1)$ storage.
    \item provide complete utility and full data availability, the query can take both the outsourced db and the data in the outsourced cache.
    \item reduce the total number of outsourced data (compare with baseline SET). The total storage equals to #record in outsourced db + cache size.
\end{itemize}

\boldparagraph{Sketch comparison}:
Given database with length $L$, and the total number of true records is $M$, where $M \leq L$
\begin{table}[]
\begin{tabular}{|l|c|l|l|}
\hline
Group   & SET & \multicolumn{1}{c|}{DP method} & \multicolumn{1}{c|}{DP + outsource cache} \\ \hline
Server Storage & $L$  &     $M + O(\frac{2\sqrt{k}}{\epsilon})$                           &      $M + O(\frac{2\sqrt{k}}{\epsilon}) + \len(\sigma)$                                     \\ \hline
%Client storage & $O(1)$  &     $k\times\len(\sigma)$                           &      $\len(\sigma)$                                     \\ \hline
\end{tabular}
\end{table}

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figure/osort.pdf}
  \caption{cache synchronization}
  \label{fig:dcache}
\end{figure}



\eat{
\boldparagraph{Sketch design}:
\begin{itemize}
    \item When system starts, the \user upload records by with SET method (ture records if received, dummy record if nothing received at that time). On the \cs, once receive record uploaded by the \user, write it to the cache (ORAM).
    \item The \user maintains a local counter $c$ to count how many records has been received between two updates and a local index ${\bf I}$ that maps the records stored in the cache.
    \item On the \cs, every time when receiving a record from the \user, the \cs appends it to the cache.
    \item When an synchronization triggers (i.e. Timer/ANT), the \user generate a random permutation based on ${\bf I}$ and ask the \cs to permute the outsourced cache. After that, the \user applies a comparison based sort to sort all records in the cache. (see figure~\ref{fig:dcache} for details).
    \item The \user then sends a noisy count $c' \gets c + Lap(\frac{1}{\epsilon})$ to the \cs. According to $c'$, read as many ``true'' records from the cache as needed ($c'$ decides it), otherwise record some dummy records to load the amount. Note that in the sorted cache, the true data will be placed on the top of dummy records. Thus the cache read should always start from the top.
\end{itemize}

\boldparagraph{Sketch comparison}:
Given database with length $L$, and the total number of true records is $M$, where $M \leq L$
\begin{table}[]
\begin{tabular}{|l|c|l|l|}
\hline
Group   & SET & \multicolumn{1}{c|}{DP method} & \multicolumn{1}{c|}{DP + outsource cache} \\ \hline
Server Storage & $L$  &     $M + O(\frac{2\sqrt{k}}{\epsilon})$                           &      $M + O(\frac{2\sqrt{k}}{\epsilon}) + \len(\sigma)$                                     \\ \hline
%Client storage & $O(1)$  &     $k\times\len(\sigma)$                           &      $\len(\sigma)$                                     \\ \hline
\end{tabular}
\end{table}

We wish that  $M + O(\frac{2\sqrt{k}}{\epsilon}) + \texup{size}(cache) < L$.  

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figure/osort.pdf}
  \caption{cache synchronization}
  \label{fig:dcache}
\end{figure}

Random permutation + sort is oblivious. The access patterns of sorting depend only
on the ranking of the records(i.e. we can set dummy records has the same, lowest ranking, and all other records will have different ranking based on their arrival time), which is independent of the input array (the record orders in the outsourced cache), after permutation.

}

}

==> revision_letter.tex <==

%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.

\begin{center}
\textbf{Revision Letter: Paper \#471 \\\appsystem: Hiding Update Patterns in Secure OutsourcedDatabases with Differential Privacy}
\end{center}


We would like to thank the reviewers for their detailed and thoughtful comments, which have helped us to significantly revise our paper in terms of completeness and readability. We have \textcolor{blue}{highlighted all new text in the main paper} for ease of reference.  The following section outlines the main changes to the paper %‚Äì (a) improved discussion on how to extend \system for the malicious adversary model, (b) experiments on larger dataset and (c) text revisions for improved paper readability
%while in Section 2, we address each reviewer's comment individually.
\subsection*{Summary of Changes}
We denote the first comment mentioned in review 1 as R1O1 and so on. All the citations in the revision letter refer to corresponding citations in the main paper. 




\stitle{Meta Review 1: Clarify the novelty and related work (R1O2)}. We have provided an expanded discussion in Section~\ref{sec:related} that highlights the differences between our work and ~\cite{agarwal2019encrypted}, ~\cite{lecuyer2019sage}, and ~\cite{kellaris2017accessing}. We describe how unlike existing work, our system efficiently tackles the problem of information leakage due to database updates where an untrusted party can look at update patterns to deduce sensitive information about data sources.  Additionally, the 1st and 4th paragraph of the original introduction highlights that the focus of this work is to protect the privacy of "when" the database is updated, which has not been addressed in previous work.  We have also pointed out that existing secure databases may fail to ensure privacy if the exact update pattern is revealed. We believe these discussions are necessary to articulate our novelty in general, thus we left these paragraphs unchanged.

\stitle{Meta Review-2: Spell out the DP privacy model, definitions and model properties (R1O1, R2O1, R2O3, R2O4, R2O5)}. We have made the following changes to address reviewers' comments. %\johes{Spell this out in the introduction as well}
\begin{itemize}
\item \textbf{(R1O1, R2O5)}: 
(i) We have improved the definition of neighboring growing databases (Definition~\ref{def:ngdb}) and further explain what they mean in practice in Section~\ref{sec:spmodel}; (ii) We improved the main privacy definition (Definition~\ref{def:dpsogdb}) and clarified that this privacy notion follows the definition of event-level DP under continual observation; (iii) To clearly explain the semantics of this privacy guarantee and to elaborate on the exact information we wish to hide, we have added a new "Privacy Semantics" section (Section~\ref{sec:semantics}) to explain the related details. In this section, we discuss the privacy semantics of Definition~\ref{def:dpsogdb} using the Pufferfish privacy framework and justify our choice of this privacy goal; (iv) Due to space constraints, we are unable to accommodate the full security proofs in the main paper, but we have provided the complete security proof in the Appendix of the full version\footnote{The anonymous full version can be accessed via \url{https://www.dropbox.com/s/ng0m4jeet3i990b/sigmod2021-paper471.pdf?dl=0}}. Note that the "sketch" proofs in the main paper contain all key steps of the full proof, such as analyzing the privacy properties of each atomic mechanism as well as the composed privacy for the entire DP strategies.

%\am{Are we including the appendix with the revision, or are we going to include a full version in an anonymous github repo?}.

\item \textbf{(R2O1)} For the discussion of principle P4 in Section~\ref{sec:ps}, we have provided an expanded description of the listed constraints with short explanations of why we need these constraints. Furthermore, since we have already discussed in detail in Section~\ref{sec:cmp} why these constraints are necessary and why some encrypted databases that do not satisfy our constraints pose certain security risks. For space reasons, we do not repeat the similar discussion in Section~\ref{sec:ps}. Instead, we added a sentence that refers the reader to Section~\ref{sec:cmp} for further details.
\item \textbf{(R2O3)}. In the conclusion, we added a short discussion on our supported database schemas. \appsystem currently only supports single table schemas. There are certain challenges to support multi-relational database schema that includes: (i) multi-relational database schema may reveal additional leakage. For example, if a database had two tables where table A held the updates satisfying condition X and table B held the other updates, then the untrusted server could deduce if an update satisfies condition X based on which table was altered. As such, handling this leakage requires additional security models and algorithms that are beyond the scope of this work; (ii) It requires an independent security protocol to calculate the sensitivity of multiple tables~\cite{johnson2018towards}, as well as data truncation techniques~\cite{kotsogiannis2019privatesql}. As such, handling this leakage requires additional security models and algorithms (i.e. secure protocols for computing sensitivity and data truncation techniques) that are beyond the scope of this work. %\nt{Shall we just say single "single table schema" and "multi-relational schema"? The description of "schema where all tables are altered on every updates seems a little bit confusing."} \am{I think we need to say clearly that we do not support multi-relational databases.}

\item \textbf{(R2O4)}. We have expanded Section~\ref{sec:updat} to explain the definition of update patterns. We also fixed typos that caused inconsistencies and added an example to further explain the concept of update pattern leakage.
\end{itemize}

\item \stitle{Meta Review-3: Motivate the privacy requirements better (R3O1, R2O6)}. To motivate the privacy requirements better, we have modified the introduction and provided a new real world privacy breach example, the main changes w.r.t. this meta review comments are listed as follows:

\begin{itemize}
\item \textbf{(R3O1)}. In the introduction, we replaced the Taxi example with a smart sensor based example, and we believe that the new example can better demonstrate the timing of an insert to the database is highly correlated with sensitive information. We also clarified our motivations in the introduction based on the new privacy breach example.

%We posit that there are several settings where the timing of an insert to the database is highly correlated with a sensitive value. This may not have been very apparent in the Taxi example we provided in the previous version of the paper \am{just say what the example is ... ``we replace the Taxi example with one based on smart sensors}. As an alternative, we replaced the Taxi example with a new real-world privacy breach example. 
\item \textbf{(R2O6)}. 
%We have provided expanded descriptions for our proposed DP strategies (Section 5.2). For each DP strategy, we added textual description of the pseudocode as well as the design logic behind them. In addition, we have already provided an overview about how different algorithm parameters would change algorithm's performance/accuracy guarantee
We have provided expanded descriptions of our proposed DP strategies (Section~\ref{sec:dps}). For each DP strategy, we added textual description of the pseudocode as well as the design logic behind them. In addition, as per how to set the algorithm parameters, it is actually highly dependent on the desired accuracy, performance and privacy goals. Since we have already provided an overview on how algorithm parameters would affect privacy/performance/accuracy guarantees in the introduction as well as provided detailed evaluations on each DP strategy with changing parameters in the experiment section (Section 8.2, 8.3). We do not repeat the similar discussion in Section 5.2 for space reasons and instead point the reader to the corresponding sections. 
%\am{SOLVED:I think you can just say what you have done and not explain why you did not do something in Sec 5.2}


%as we have already provided detailed experiments on how different algorithm parameters ($\epsilon, \theta, T$) would affect the accuracy and performance guarantees (Section 8.2, 8.3). Thus we do not repeat the similar discussion in Section 5.2 and instead point the reader to the corresponding sections. 
%Moreover, we believe the reader can better understand how to set these parameters under different accuracy or performance goals as well as their trad-offs after seeing the experiment results.
\end{itemize}
%\item \stitle{Other changes}:
%To comply with formatting requirements, we have removed all appendices from the manuscript and attached them to this revision letter. In addition, for ease of reviewing, we have uploaded an anonymous full version manuscript with complete appendices.

\stitle{Other changes}. Some other changes in addition to the meta review comments are summarized as follows:\vspace{-1mm}
\begin{itemize}
    \item To comply with the SIGMOD21 paper format guideline, we have removed the appendix from our submitted manuscript. We have uploaded an anonymous full version separately with the complete appendix attached. The anonymous full version can be found at:\\\textcolor{blue}{ \url{https://www.dropbox.com/s/ng0m4jeet3i990b/sigmod2021-paper471.pdf?dl=0}}
    
    \item We fixed all typos and improved some descriptions to make them more rigorous.
    
    
    
\end{itemize}


\subsection*{Individual Reviewer Comments}
%We now directly address reviewer‚Äôs comments,
In this section, we respond to individual reviewers' comments. Note that when directly quoting reviewers comments, we will be using \textit{italic type font}. 
\eat{
\subsubsection{Meta Review Comments}
\textit{1. Clarify the novelty and related work}. \\
We have added discussions in Section~\ref{sec:intro} and Section~\ref{sec:related} that clarify the novelty of our work in the context of prior work. We discuss how while previous work focused on information leakage due to query outputs, \appsystem is the first system to consider information leakage due to database updates. We include a real-world example in Section~\ref{sec:intro} that shows why and how update patter leakage can compromise sensitive information.


\noindent\textit{2. Spell out the DP privacy model, definitions and model properties}. \\
We have clarified in Section~\ref{sec:spmodel} that the definition of our DP privacy model is analogous to event-level DP and have provided more rigorous definitions (Definition 2, 4, 5). We have also improved the description of the neighboring growing databases and added discussion about what they mean in practice. To better interpret our privacy guarantee, and to elaborate what exact information we wish to hide from the adversary, we added a new section "Privacy Semantics" (section 4.4) to further discuss the related details. In this section, we utilize Pufferfish framework and explored the privacy semantics behind Definition 5 from the perspective of disclosing secrets to adversaries. In addition, we also revised the introduction and spelled out our DP privacy model.\\ 

\noindent\textit{3. Motivate the privacy requirements better}\\
 We have provided an new real world privacy breach example in the introduction which can demonstrate that the timing of an insertion to the database would reveal sensitive information. We also improved the related discussion in the introduction to motivate the privacy requirements better. Moreover, we have enriched the description of our proposed DP strategies (Section 5.2) by adding textual descriptions of the pseudocode, as well as discussing the design logic behind the two DP strategies.
 }

%\subsubsection{Individual Review Comments}
\\
\boldparagraph{Reviewer \#1}\\
\noindent\textit{R1O1. There are no rigorous definitions for what type of DP they are using, it seems to be event based DP, but they do not clarify or introduce the different notions for continual observation, which one they use and why, or what exactly they are trying to hide (e.g., a single user transaction? a user? a user throughout time?). There is a need for a definition of neighboring DBs and what they mean in practice in order to understand the sensitivity they define. Also, the DP proofs would be better to be actual proofs and not sketches.}\\

We have improved the related content in Section~\ref{sec:spmodel} as follows: (i) We have clarified that our DP model is analogous to event-level privacy as defined in~\cite{dwork2010differential}. (ii) We also provided an expanded description of neighboring growing database and have discussed what they mean in practice. (iii) In general, we focus on hiding the presence or absence of a single record (i.e. a single transaction or event w.r.t. a single user) in the database over time. To further elaborate what exact information we wish to hide from the adversary, we have provided a "Privacy Semantics" section that explores the semantics behind our privacy notion. (iv) We also provide a complete security proof in the Appendix of the full version\footnote{The anonymous full version can be accessed via \url{https://www.dropbox.com/s/ng0m4jeet3i990b/sigmod2021-paper471.pdf?dl=0}}, however we're unable to accommodate this full proof in the main content. But please note that, the "sketch" proofs we provided in the main content covers all key steps of the full proofs, such as analyzing the privacy of each atomic mechanisms as well as the composed privacy for the entire DP strategy.\\
%\johes{Write out the rebuttal for each specific reviewer}
%\johes{Include proofs in full version and put in anonymous dropbox}

 
\textit{R1O2. There is a question about the novelty. The related work is not well described as to how their methods differ from~\cite{agarwal2019encrypted}, ~\cite{lecuyer2019sage}, and ~\cite{kellaris2017accessing}.}\\

We revised the related work (Section~\ref{sec:related}) and have provided an expanded discussion to compare our work with~\cite{agarwal2019encrypted},~\cite{lecuyer2019sage}, and~\cite{kellaris2017accessing}. Agarwal et al.~\cite{agarwal2019encrypted} consider the problem to release DP queries over dynamic encrypted databases, their work focus on hiding the query protocol leakage and guarantees that any adversary can learn from the query protocol is bounded by DP. However, they did not consider hiding the update leak, which is the focus of our work. Lécuyer et al.~\cite{lecuyer2019sage} proposed an private ML model update strategy with growing training dataset. Their work guarantees that, each time when the model has updated, the adversary can not infer useful information against the newly added training data by observing the model changes. 
However, they do not consider the update pattern (related to the amount of each update) as well. Thus, if the adversary can monitor the traffic between the server and the client, such an adversary can still obtain critical information about the training data even without access to the ML models.  Kellaris et al~\cite{kellaris2017accessing}. mentioned to distort the amount of updates, but their method always overcounts the number of records in each update, which contains a large number of dummy records. Moreover, none of these works have tried to formulate the update pattern leakage as well as it's corresponding privacy or design private synchronization strategies to hide the update pattern.\\
%\am{SOLVED:Do we need () in the previous sentence?}
 
 
\boldparagraph{Reviewer \#2}\\

\textit{R2O1. Page 3, Section 2: In the discussion of principle P4, the authors list the constraints that should be satisfied by the encrypted databases to support the proposed framework. It would be beneficial for the reader to see an intuitive explanation of the motivations for having these constraints. I would suggest the authors to enrich the description with such explanations.}\\

We have made changes according to the reviewer's suggestion and revised the discussion of P4. In the revised discussion, we list our constraints with short explanations of why we consider these constraints. In addition, since we have a separate section (Section~\ref{sec:cmp}) that discusses in detail why some encrypted databases that do not satisfy our constraints pose certain security risk. Therefore, we do not repeat the full discussion in Section 2 for space reasons. Instead, we added a sentence that refers the reader to Section~\ref{sec:cmp} for further information.\\

\textit{R2O3. Page 4, Section 4.1: Can the database be composed of multiple tables? In this case, what does the insertion of a record represent? Is it possible to consider the addition of multiple records in different tables? What happens if such records are somehow dependent one from the other?}\\
%\nt{This response is related to the multiple case, need to check whether it is consistent with our revisions.}

We have added a short discussion of the schemas supported by our system in the Conclusion. Currently, \appsystem only supports single table schema. Support for multi-relational table databases requires additional security models, as multi-relational table databases may expose additional leakage. For example, if a database had two tables where table A held the updates satisfying condition X and table B held the other updates, then the untrusted server could deduce if an update satisfies condition X based on which table was altered. Additionally, a separate security protocol is required to calculate sensitivity across multiple tables~\cite{johnson2018towards} as well as to apply some data truncation techniques~\cite{kotsogiannis2019privatesql}, which are beyond the scope of this work. Therefore, we leave the design that handles multi-relational table databases for future works.\\
\eat{
In the conclusion, we added a short discussion on our supported database schemas. \appsystem currently only supports single table schemas. There are certain challenges to support multi-relational database schema that includes: (i) multi-relational database schema may reveal additional leakage. For example, if a database had two tables where table A held the updates satisfying condition X and table B held the other updates, then the untrusted server could deduce if an update satisfies condition X based on which table was altered. (ii) It requires an independent security protocol to calculate the sensitivity of multiple tables~\cite{johnson2018towards}, as well as data truncation techniques~\cite{kotsogiannis2019privatesql}. As such, handling this leakage requires additional security models and algorithms (i.e. secure protocols for computing sensitivity and data truncation techniques) that are beyond the scope of this work.
We have added a short discussion of the schemas supported by our system in Section~\ref{sec:cmp}. A database can be composed multiple tables as long as a single update alters all tables, where one table receives the encrypted record and any other tables receive an encrypted dummy record. This prevents the server from learning information about the update based on which tables are updated
If not all tables are altered on every update, then the set of altered tables leaks information about the update. For example, if a database had two tables where table A held the updates satisfying condition X and table B held the other updates, then the untrusted server could deduce if an update satisfies condition X based on which table was altered. As such, handling this leakage requires additional security models and algorithms that are beyond the scope of this work} 

\textit{R2O4. Page 5, Section 4.2: The update pattern is a key definition for the proposed approach. I therefore suggest the authors to better clarify it, also possibly showing an example. 
owing: 1) the relationship between j and t in the definition of $UpdtPatt_t(D_t)$; and 2) the meaning of L’.}\\

We have made revisions of Section~\ref{sec:updat} according to the reviewer's suggestion. We have provided an improved definition for update pattern followed by an example, we also fixed all typos that caused inconsistencies.\\


\textit{R2O5. Page 5, Section 4.3: The authors should better explain the security model and the intuition behind it. Why does Definition 4 ensure the protection of the update pattern? What is $\Sigma$? Why the UpdtPatt in Definition 4 has two arguments ($\Sigma$ and $D$) and UpdtPatt in Section 4.2 has one argument only $(D_t)$? What is the intuition behind $L_U$?}\\

We have improved our main privacy definition (Definition 5) and fixed all typos that causes inconsistencies. In addition, to better explain the intuition behind this privacy notion, we have added a new section "Privacy Semantics" (Section~\ref{sec:semantics}) to further explore the privacy semantics guaranteed by Definition 5. In this section, we utilize the Pufferfish framework and interpret the privacy semantics in terms of the secret disclosed to the adversaries.\\


\textit{R2O6. Page 6, Section 5.1: Since the naive strategies does not satisfy the principles discussed in Section2, what is the rationale for presenting and comparing them with the DP strategies (Section 8.1)? The authors should consider the possibility of removing the description of such naive strategies in favor of improving the description of the two proposed DP strategies. For instance, aspects that could be improved are: 1) the textual description of the pseudocode of Algorithms 1-3, which is now missing; 2) the description of the rationale behind the proposed strategies, possibly with some simple examples; 3) the description of the different parameters that characterize the proposed strategies (not only $T$ and $\theta$), how they are set, and their impact on the DP strategies.}\\

We have provided a more detailed description of the proposed DP strategies (Section~\ref{sec:dps}). For each DP strategy, we added textual description of the pseudocode as well as the design logic behind them. In addition, since we have already provided an overview on how algorithm parameters would affect it's corresponding performance and accuracy guarantee in the introduction as well as detailed evaluations on each DP strategy with changing parameters in the experiment section (Section 8.2, 8.3). Thus we believe with such contents, the reader can get a better understand on how to set these parameters under different accuracy or performance goals as well as their trade-offs. Hence, we do not repeat the similar discussion in Section~\ref{sec:dps} and instead point the reader to the corresponding sections. 

%Moreover, we believe the reader can better understand how to set these parameters under different accuracy or performance goals as well as their trade-offs after seeing the experiment results.

\boldparagraph{Reviewer \#3}\\
\textit{R3O1. In general, I find it difficult to understand why record insertion time could really reveal sensitive information. One may argument that update patterns are also a type of access patterns, and it is known that access patterns could reveal information about the data. However, conventional access patterns (namely, read/write sequences) are revealing only because they might be dependent on the information in the data; in contrast, the record insertion time does not really depend on sensitive information in the record, so I do not see why it cannot be known by the cloud server. The paper should be revised to provide more convincing motivation of the problem..}\\

We posit that there are several settings where the timing of an insert to the database is highly correlated with a sensitive value. This may not have been very apparent in the Taxi example we provided in the introduction. As an alternative, we have include a new smart sensor based example which better demonstrates how the timing of updates can disclose sensitive properties. Moreover, to better motivate the privacy requirements, we also improved the related discussion in the introduction after the new privacy breach example.

\pagebreak

